FlowControl: Optical Flow Based Visual Servoing

One-shot imitation is the vision of robot programming from a single demonstration, rather than by tedious construction of computer code. We present a practical method for realizing one-shot imitation for manipulation tasks, exploiting modern learning-based optical flow to perform real-time visual servoing. Our approach, which we call FlowControl, continuously tracks a demonstration video, using a specified foreground mask to attend to an object of interest. Using RGB-D observations, FlowControl requires no 3D object models, and is easy to set up. FlowControl inherits great robustness to visual appearance from decades of work in optical flow. We exhibit FlowControl on a range of problems, including ones requiring very precise motions, and ones requiring the ability to generalize.

==> scap_algo.tex <==
\begin{algorithm}[htb]
 \KwData{demo. observations and segmentations $O^{D}, S^{D}$ \\ live observations $O^L$, and distance threshold $\delta$}
 \KwResult{imitated interaction }
 \setstretch{1.1}
 t = 0 \tcp*{demo. frame index}
 \While{$t < T$}{
 $T = \text{FrameAlign}(O_t^D, S_t^D, O^L)$\tcp*{3D trnf.}
 \eIf{ $|T| > \delta$}{
 $a_t = a(O_t^D, T)$\tcp*{choose action act}
 }{
 $t=t+1$\tcp*{incr. demo. frame}
 }
 }
 \caption{\textbf{Sequence Tracking}: Continuously align, when close enough continue to next demonstration frame.}
 \label{alg:sequence_track}
\end{algorithm}


==> scrap_christians_into.tex <==

%\section*{Organization}
%Papers should be six pages in length, with up to two extra pages at the cost of US$180$ per extra page. A short video (1-minute %maximum) can also be sent later on, attached to your paper. --ICRA 2019

%\Max{desired reviewers: RL/VS/Flow/Vision? diction.}\\
%Length: 6+2 pages incl. citations and 1 min video.

%\begin{enumerate}
%    \item our approach generalizes because of flow
%    \item highlight differences (data efficiency + req. )
%    \item our method is practical
%\end{enumerate}

\iffalse
\section{Christians' Introduction}

% Motivation 
Teaching robots a new task is a central problem of robotics and various approaches were proposed for it. Especially industry is showing an increasing interest to quickly teach robots new tasks. This allows to use expensive machinery across a much broader spectrum of tasks and allows for larger flexibility. 

% Problems, Challenges
%Different approaches to the task learning problem are facing different challenges. 
%Programming
Historically, an expert explicitly formulates the robot task in a computer program executed by the robot. This method is heavily used in the large throughput industrial sector, yet it is not an option for unlearned personnel or consumers.

%L-by-D
In the learning from demonstration setting, the robot perceives the new task and learns how to imitate movements and actions. This is achieved either by kinesthetic teaching, which requires an instructor to physically move the robots actuators, or by a high level of perceptual understanding of its surrounding environment. Both approaches usually need multiple demonstrations. The learned model tends to replicate the demonstrations very closely, which usually leads to a low level of robustness with respect to variations in the task setup. 

%Reinforement Learning
Recently, reinforcement learning (RL) has gained popularity for learning complex tasks. RL comes with the attractive promise to generalize over variations in the environment and the robot's parameters. However, many trials are needed before even a simple task is learned. Therefore, most research is done in simulated environments. Due to the gap between simulation and the real world, only few works can show successful transfer to a real robotic system. 

% Our contribution
In this paper, we propose a one-shot imitation learning approach, which can robustly replicate a task from a single demonstration video. We formulate the task as correspondence problem: given a state from the demonstration, we find correspondences towards the currently observed state of the robot, and deduct the necessary action to align the two. Hereby, we leverage recent advances in optical flow estimation, which provide robust methods to find correspondences, and build a visual servoing loop on top. Whenever a demonstration state is reached, the target demonstration is advanced in time. This formulation naturally extends to multi-step tasks and does neither require CAD models of the manipulated objects, nor expensive pre-training in elaborate simulation environments.

% Experimental results
Despite its simplicity, this approach shows a large degree of robustness towards various factors of variation. Experiments show task learning for a variety of tasks that require precise control with high success rates. %being both data efficient and operating at a higher success rate. The high performance paired with the easy applicability makes our approach a practical and viable way for robotic learning in the future.
\fi
